SNED: Superposition Network Architecture Search for Efficient Video Diffusion Model

While AI-generated content has garnered significant attention, achieving photo-realistic video synthesis remains a formidable challenge. Despite the promising advances in diffusion models for video generation quality, the complex model architecture and substantial computational demands for both training and inference create a significant gap between these models and real-world applications. This paper presents SNED, a superposition network architecture search method for efficient video diffusion model. Our method employs a supernet training paradigm that targets various model cost and resolution options using a weight-sharing method. Moreover, we propose the supernet training sampling warm-up for fast training optimization. To showcase the flexibility of our method, we conduct experiments involving both pixel-space and latent-space video diffusion models. The results demonstrate that our framework consistently produces comparable results across different model options with high efficiency. According to the experiment for the pixel-space video diffusion model, we can achieve consistent video generation results simultaneously across 64 x 64 to 256 x 256 resolutions with a large range of model sizes from 640M to 1.6B number of parameters for pixel-space video diffusion models.

==> sec/rebuttal-v2.tex <==
Thank all reviewers for their thoughtful comments. Please find our responses to each reviewer as follows. Please also make sure to check the previous supplementary material for the demo and more results comparisons.

% \noindent\textbf{\rbt{Reviewer P379}}

% \noindent\textbf{\rbt{Q1} Why use NAS not directly train a model?}
% We use NAS mainly based on these three reasons: Training in video diffusion models is expensive. Besides that, traditional model architecture design highly relies on try-and-error. If we want to obtain models with different sizes and resolutions for different situations, we need to repeat and try the training again and again which incurs a huge total consumption. By using our proposed SNED, we can achieve multiple models with different model sizes and resolutions at the same time to save the training costs.
% Please also check our PSDM result shown in the supplementary material.

\noindent\textbf{\rbt{(P379) Q1:} Why opt for NAS instead of direct model training?}
NAS is chosen for three main reasons: 1) Video diffusion model training is resource-intensive. 2) Conventional model design relies heavily on trial-and-error, leading to repetitive training for diverse sizes and resolutions. 3) Our proposed SNED allows simultaneous training of multiple models, reducing overall training costs. Refer to supplementary material for PSDM results, we achieve multiple small-size models with a similar level of evaluation score.



\noindent\textbf{\rbt{Q2:} Comparisons with models with specific model size.  }
Thanks for your advice. Using LVDM as an example, we decrease the number of channels in each layer to 75\%, train the whole model with the same hyper-parameters, and then evaluate the model using the same strategy as shown in Section 4.4.3. The shrunk model number of parameters, KVD, and FVD scores are 411 M, 410.8, and 30.9, respectively. Compared with our SNED model with the same model size, we achieve better FVD and KVD scores of 348.2 and 23.5. More experiments for the same model size comparisons will be added to the revision.

% and compared with our SNED subnet

% \begin{table}[h] 
% \centering
% \scalebox{0.8}{
% \begin{tabular}{c|cccc}
% \toprule
%  Model & \#Params (M) & $FVD\downarrow$  & $KVD\downarrow$   \\ 

% \midrule
% LVDM-75\% & 411 & 410.8 & 30.9 \\
% SNED & 411 & 348.2 & 23.5  \\
% LVDM-50\% & 274 & -  & - \\
% SNED & 274 & 472.3  & 28.7     \\
% \bottomrule
% \end{tabular}}
% \end{table}

\noindent\textbf{\rbt{Q3:} Comparison with other NAS.} 
To the best of our knowledge, this is the first NAS framework targeting video diffusion models. So we didn't provide NAS comparisons. 

% \noindent\textbf{\rbt{Reviewer hPQB}}

\noindent\textbf{\rbt{(hPQB) Q1:} EMA and initializing spatial model weights with pre-trained images diffusion model weights have already been studied.  } 
Yes, these two are not part of our novalties but just part of the optimization. We will move them into the appendix for the revision.


\noindent\textbf{\rbt{Q2:} Ablation study for supernet training sampling warmup (STSW).  } 
Thanks for your advice. Here we attach our ablation study on PSDM for different sizes of subnets:
\begin{table}[h] 
\centering
\scalebox{0.8}{
\begin{tabular}{c|cccccc}
\toprule
\multirow{2}*{\textbf{Model}}  & \multirow{2}*{\textbf{\#Params (B)}}   & \multicolumn{2}{c}{\textbf{W/ STSW} } & \multicolumn{2}{c}{\textbf{W/O STSW} }  \\ 
& & \textbf{FVD$\downarrow$} & \textbf{KVD$\downarrow$} & \textbf{FVD$\downarrow$} & \textbf{KVD$\downarrow$}\\

\midrule
% SNED-B & 1.60 & 544.4 & 25.8 & 510.9 & 19.4\\
SNED-L & 1.28 & \textbf{490.5} & \textbf{13.0}  & 516.7 & 19.9\\
SNED-M & 0.96 & \textbf{452.2}  & \textbf{14.4} & 517.4 & 18.8\\
SNED-S & 0.64 & \textbf{472.3}  & \textbf{16.8} & 515.5 & 19.9 \\
\bottomrule
\end{tabular}}
\end{table}

Training with STSW consistently yields superior scores for both FVD and KVD in comparison to not using it.

% \noindent\textbf{\rbt{Q3:} Prove "optimizing the model's resource allocation". Show training consumption for Table 1. } 
% Thanks for your question. Here "optimizing the model's resource allocation" only means we can search models with fewer parameters with good generation quality. In Appendix Table 1, we obtain models with 1.28 B, 0.96 B, and 0.64 B parameters with 21.2 s, 18.1 s, and 16.0 s inference time, respectively. Compared with the base model, these three models achieve 80\%, 60\%, and 40\% smaller model sizes with the same level of evaluation score. We will modify our illustration to prevent ambiguity.
% For Table 1, we use similar settings to align with LVDM~\cite{he2022latent} (200 epochs) as shown in Section 4.1. After one term of training, we get all the models shown in Table 1. The total GPU memory consumption is slightly larger than directly training a full-size LVDM model.

\noindent\textbf{\rbt{Q3:} Prove "optimizing the model's resource allocation." Show training consumption for Table 1.}

"Optimizing the model's resource allocation" implies training models for different sizes and resolutions with weight sharing. In Appendix Table 1, we obtained models with 1.6 B, 1.28 B, 0.96 B, and 0.64 B parameters in one term of training by allocating only the 1.6 B model. If we train them in parallel, the total allocated model size will be 4.48 B. We will modify our illustration to prevent ambiguity. For Table 1, our settings align with LVDM~\cite{he2022latent} (200 epochs) in Section 4.1. After one training term, all Table 1 models are obtained, with a GPU memory consumption slightly larger than directly training a full-size LVDM (around 39 GB per GPU for 32 batch size). 
% Please also check the demo in the previous supplementary material for the resolution comparison.



\noindent\textbf{\rbt{Q4:} Meaning of model efficiency.} 
 Efficiency here means both less memory consumption and inference/training time. From experimental results (Table 1 in the main content and Table 1 in the Appendix) we can see that, our approach can obtain many models with smaller model sizes (less memory consumption) and shorter model latency (less inference time) in one term of training. All models can be trained simultaneously rather than sequentially, resulting in significant time savings (less training time).



% \noindent\textbf{\rbt{Q5:} Explain the following terms:}
% 1) One-shot superposition NAS method: The One-Shot NAS method entails training a singular network that encompasses a multitude of potential architectures. The term "superposition" refers to the sharing of weights among models for various resolutions, where the weights of models at different resolutions are "superposed" upon each other.
% 2) Supernet training sampling warmup: As shown in Section 3.4, it means that we gradually increase our search space during the training, rather than directly applying a full random subnet sampling among the whole search space at the beginning. For instance, in the beginning, we only train the full model, after several iterations, we start to enable sampling 90\%-channel subnets for training. Subsequently, additional increments from 80\% to 40\% are sequentially integrated into our expanding search space. This stepwise warmup strategy enhances the stability of the Supernet training.
% 3) Image-based diffusion model transfer learning: it means initializing spatial model weights with pre-trained image-based diffusion model weights for training.
% Thank you for pointing these out, we will refine our explanation of them in the revision.

\noindent\textbf{\rbt{Q5:} Explain the following terms:}
1) \textbf{One-Shot Superposition NAS Method:} A singular network is trained to encompass various potential architectures. "Superposition" denotes weight sharing among models for different resolutions, where weights from models at distinct resolutions are "superposed" upon each other.
2) \textbf{Supernet Training Sampling Warmup:} In Section 3.4, this involves a gradual expansion of the search space during training, as opposed to an initial full random subnet sampling. Using channel space as an example: initially, only the full model is trained. Subsequently, sampling subnets from 90\% to 40\% channels for each layer are sequentially integrated into the search space. 
This stepwise warmup strategy enhances Supernet training stability.
3) \textbf{Image-based Diffusion Model Transfer Learning:} This term refers to initializing spatial model weights with pre-trained weights from an image-based diffusion model for training. Thank you for your feedback. We will refine these explanations in the revision.

% \noindent\textbf{\rbt{Reviewer nJgy}}

\noindent\textbf{\rbt{(nJgy) Q1:} Why not use resizing instead of multi-resolution diffusion models?}
This is because directly generating high-resolution videos requires higher computation costs. In scenarios where lower resolutions are sufficient, we want to reduce the overall computational expenses. Small-resolution subnets can be used independently.


\noindent\textbf{\rbt{Q2:} Change the illustration of L197-198; add real-resolution images to Fig.3; modify typos.}
Thanks for your advice! We will modify them in the revision. 

\noindent\textbf{\rbt{Q3:} Detailed comparisons for the visualization in the text for Fig.5. }
We observe that samples produced by both LVDM and SNED have high fidelity and diversity, including different skies, clouds, and ground at different times of the day. We will add more comparisons in the revision.

\noindent\textbf{\rbt{Q4:} Training performance comparison.} 
Our strategy improves the training performance in two dimensions: 1) Shorter total training time: we can obtain a large range of models for different sizes and resolutions at the same time, which offers a substantial increase in time efficiency proportional to the number of different required models. 2) Better generation quality. Please check Q2 for reviewer hPQB to see the ablation study for the proposed STSW strategy.




==> sec/rebuttal.tex <==
Thank all reviewers for their thoughtful comments. Please find our responses to each reviewer as follows. Please also make sure to check the previous supplementary material for the demo and more results comparisons.

% \noindent\textbf{\rbt{Reviewer P379}}

% \noindent\textbf{\rbt{Q1} Why use NAS not directly train a model?}
% We use NAS mainly based on these three reasons: Training in video diffusion models is expensive. Besides that, traditional model architecture design highly relies on try-and-error. If we want to obtain models with different sizes and resolutions for different situations, we need to repeat and try the training again and again which incurs a huge total consumption. By using our proposed SNED, we can achieve multiple models with different model sizes and resolutions at the same time to save the training costs.
% Please also check our PSDM result shown in the supplementary material.

\noindent\textbf{\rbt{(P379) Q1:} Why opt for NAS instead of direct model training?}
NAS is chosen for three main reasons: 1) Video diffusion model training is resource-intensive. 2) Conventional model design relies heavily on trial-and-error, leading to repetitive training for diverse sizes and resolutions. 3) Our proposed SNED allows simultaneous training of multiple models, reducing overall training costs. Refer to supplementary material for PSDM results, we achieve multiple small-size models with a similar level of evaluation score.



\noindent\textbf{\rbt{Q2:} Comparisons with the specific model size.  }

Thanks for your advice. Using LVDM as an example, we decrease the number of channels in each layer to 50\% and 75\% then train them with the same hyper-parameters. Here we attach our ablation study as follows:

\begin{table}[h] 
\centering
\scalebox{0.8}{
\begin{tabular}{c|cccc}
\toprule
 Model & \#Params (M) & $FVD\downarrow$  & $KVD\downarrow$   \\ 

\midrule
LVDM-75\% & 411 & 410.8 & 30.9 \\
SNED & 411 & 348.2 & 23.5  \\
LVDM-50\% & 274 & -  & - \\
SNED & 274 & 472.3  & 28.7     \\
\bottomrule
\end{tabular}}
\end{table}

\noindent\textbf{\rbt{Q3:} Comparison with other NAS.} 
To the best of our knowledge, this is the first NAS framework targeting video diffusion models. So we didn't provide NAS comparisons. 

% \noindent\textbf{\rbt{Reviewer hPQB}}

\noindent\textbf{\rbt{(hPQB) Q1:} EMA and initializing spatial model weights with pre-trained images diffusion model weights have already been studied.  } 
Yes, these two are not part of our novalties but just part of the optimization. We will move them into the appendix for the revision.


\noindent\textbf{\rbt{Q2:} Ablation study for supernet training sampling warmup (STSW).  } 
Thanks for your advice. Here we attach our ablation study on PSDM for different sizes of subnets:
\begin{table}[h] 
\centering
\scalebox{0.8}{
\begin{tabular}{c|cccccc}
\toprule
\multirow{2}*{\textbf{Model}}  & \multirow{2}*{\textbf{\#Params (B)}}   & \multicolumn{2}{c}{\textbf{W/ STSW} } & \multicolumn{2}{c}{\textbf{W/O STSW} }  \\ 
& & \textbf{FVD$\downarrow$} & \textbf{KVD$\downarrow$} & \textbf{FVD$\downarrow$} & \textbf{KVD$\downarrow$}\\

\midrule
% SNED-B & 1.60 & 544.4 & 25.8 & 510.9 & 19.4\\
SNED-L & 1.28 & \textbf{490.5} & \textbf{13.0}  & 516.7 & 19.9\\
SNED-M & 0.96 & \textbf{452.2}  & \textbf{14.4} & 517.4 & 18.8\\
SNED-S & 0.64 & \textbf{472.3}  & \textbf{16.8} & 515.5 & 19.9 \\
\bottomrule
\end{tabular}}
\end{table}

Training with STSW consistently yields superior scores for both FVD and KVD in comparison to not using it.

% \noindent\textbf{\rbt{Q3:} Prove "optimizing the model's resource allocation". Show training consumption for Table 1. } 
% Thanks for your question. Here "optimizing the model's resource allocation" only means we can search models with fewer parameters with good generation quality. In Appendix Table 1, we obtain models with 1.28 B, 0.96 B, and 0.64 B parameters with 21.2 s, 18.1 s, and 16.0 s inference time, respectively. Compared with the base model, these three models achieve 80\%, 60\%, and 40\% smaller model sizes with the same level of evaluation score. We will modify our illustration to prevent ambiguity.
% For Table 1, we use similar settings to align with LVDM~\cite{he2022latent} (200 epochs) as shown in Section 4.1. After one term of training, we get all the models shown in Table 1. The total GPU memory consumption is slightly larger than directly training a full-size LVDM model.

\noindent\textbf{\rbt{Q3:} Prove "optimizing the model's resource allocation." Show training consumption for Table 1.}

"Optimizing the model's resource allocation" implies training models for different sizes and resolutions with weight sharing. In Appendix Table 1, we obtained models with 1.6 B, 1.28 B, 0.96 B, and 0.64 B parameters in one term of training by allocating only the 1.6 B model. If we train them in parallel, the total allocated model size will be 4.48 B. We will modify our illustration to prevent ambiguity. For Table 1, our settings align with LVDM~\cite{he2022latent} (200 epochs) in Section 4.1. After one training term, all Table 1 models are obtained, with a GPU memory consumption slightly larger than directly training a full-size LVDM. 
% Please also check the demo in the previous supplementary material for the resolution comparison.



\noindent\textbf{\rbt{Q4:} Meaning of model efficiency.} 
 Efficiency here means both less memory consumption and inference/training time. From experimental results (Table 1 in the main content and Table 1 in the Appendix) we can see that, our approach can obtain many models with smaller model sizes (less memory consumption) and shorter model latency (less inference time) in one term of training. All models can be trained simultaneously rather than sequentially, resulting in significant time savings (less training time).



% \noindent\textbf{\rbt{Q5:} Explain the following terms:}
% 1) One-shot superposition NAS method: The One-Shot NAS method entails training a singular network that encompasses a multitude of potential architectures. The term "superposition" refers to the sharing of weights among models for various resolutions, where the weights of models at different resolutions are "superposed" upon each other.
% 2) Supernet training sampling warmup: As shown in Section 3.4, it means that we gradually increase our search space during the training, rather than directly applying a full random subnet sampling among the whole search space at the beginning. For instance, in the beginning, we only train the full model, after several iterations, we start to enable sampling 90\%-channel subnets for training. Subsequently, additional increments from 80\% to 40\% are sequentially integrated into our expanding search space. This stepwise warmup strategy enhances the stability of the Supernet training.
% 3) Image-based diffusion model transfer learning: it means initializing spatial model weights with pre-trained image-based diffusion model weights for training.
% Thank you for pointing these out, we will refine our explanation of them in the revision.

\noindent\textbf{\rbt{Q5:} Explain the following terms:}
1) \textbf{One-Shot Superposition NAS Method:} A singular network is trained to encompass various potential architectures. "Superposition" denotes weight sharing among models for different resolutions, where weights from models at distinct resolutions are "superposed" upon each other.
2) \textbf{Supernet Training Sampling Warmup:} In Section 3.4, this involves a gradual expansion of the search space during training, as opposed to an initial full random subnet sampling. Using channel space as an example: initially, only the full model is trained. Subsequently, sampling subnets from 90\% to 40\% channels for each layer are sequentially integrated into the search space. 
% This stepwise warmup strategy enhances Supernet training stability.
3) \textbf{Image-based Diffusion Model Transfer Learning:} This term refers to initializing spatial model weights with pre-trained weights from an image-based diffusion model for training. Thank you for your feedback. We will refine these explanations in the revision.

% \noindent\textbf{\rbt{Reviewer nJgy}}

\noindent\textbf{\rbt{(nJgy) Q1:} Why not use resizing instead of multi-resolution diffusion models?}
This is because directly generating high-resolution videos requires higher computation costs. In scenarios where lower resolutions are sufficient, we want to reduce the overall computational expenses. Small-resolution subnets can be used independently.


\noindent\textbf{\rbt{Q2:} Change the illustration of L197-198; add real-resolution images to Fig.3; modify typos.}
Thanks for your advice! We will modify them in the revision. 

\noindent\textbf{\rbt{Q3:} Detailed comparisons for the visualization in the text for Fig.5. }
We observe that samples produced by both LVDM and SNED have high fidelity and diversity, including different skies, clouds, and ground at different times of the day. We will add more comparisons in the revision.

\noindent\textbf{\rbt{Q4:} Training performance comparison.} 
Our strategy improves the training performance in two dimensions: 1) Shorter total training time: we can obtain a large range of models for different sizes and resolutions at the same time, which offers a substantial increase in time efficiency proportional to the number of required models. 2) Better generation quality. Please check Q2 for reviewer hPQB to see the ablation study for the proposed STSW strategy.



